A machine learning approach to portfolio pricing and risk management for high-dimensional problems

We present a general framework for portfolio risk management in discrete time, based on a replicating martingale. This martingale is learned from a finite sample in a supervised setting. The model learns the features necessary for an effective low-dimensional representation, overcoming the curse of dimensionality common to function approximation in high-dimensional spaces. We show results based on polynomial and neural network bases. Both offer superior results to naive Monte Carlo methods and other existing methods like least-squares Monte Carlo and replicating portfolios.

==> comparison_lasso_call.tex <==
% lasso_comparison generated:  2020-12-18 16:48:45.358619
\begin{tabular}{@{}rrrrrrrrrrr@{}}
\toprule
& \multicolumn{3}{r}{\textbf{MApE ES}} & \multicolumn{3}{r}{\textbf{Rel. mean L\textsubscript{1} error}} \\
\textbf{\textbf{Samples}} &            Lasso &  LDR & N. Net. &                                       Lasso & LDR & N. Net. \\
\midrule
\multicolumn{1}{l}{\textbf{\textbf{\textbf{T}}=5}}  &   &   &   &   &   &   \\
                    1,000 &             24.1 &  2.0 &     0.9 &                                         8.4 & 1.1 &     0.5 \\
                    5,000 &              8.8 &  0.9 &     0.2 &                                         2.6 & 0.6 &     0.4 \\
                   10,000 &              7.3 &  0.7 &     0.1 &                                         2.2 & 0.6 &     0.4 \\
                   50,000 &              1.7 &  0.5 &     0.0 &                                         0.9 & 0.5 &     0.4 \\
\multicolumn{1}{l}{\textbf{\textbf{\textbf{T}}=40}}  &   &   &   &   &   &   \\
                    1,000 &            100.0 & 10.0 &    16.0 &                                        64.2 & 4.6 &     7.4 \\
                    5,000 &             83.9 &  6.5 &     4.9 &                                        24.7 & 2.6 &     2.2 \\
                   10,000 &             70.8 &  4.9 &     3.3 &                                        17.9 & 2.0 &     1.4 \\
                   50,000 &                &  2.9 &     1.0 &                                           & 1.3 &     0.8 \\
\bottomrule
\end{tabular}

==> nMC_pv_comparison.tex <==
% nMC_pv_comparison generated:  2020-05-08 11:00:18.673116
\begin{tabular}{@{}rrrr@{}}
\toprule
 \textbf{Maturity} & \textbf{Benchmark} & \textbf{nMC} & \textbf{MApE} \\
\midrule
                 5 &            22.1691 &      22.1806 &         0.6\% \\
                40 &            67.5488 &      67.5567 &         1.0\% \\
\bottomrule
\end{tabular}
